Efficient and Robust Distributed Matrix Computations via Convolutional Coding

Distributed matrix computations -- matrix-matrix or matrix-vector multiplications -- are well-recognized to suffer from the problem of stragglers (slow or failed worker nodes). Much of prior work in this area is (i) either sub-optimal in terms of its straggler resilience, or (ii) suffers from numerical problems, i.e., there is a blow-up of round-off errors in the decoded result owing to the high condition numbers of the corresponding decoding matrices. Our work presents convolutional coding approach to this problem that removes these limitations. It is optimal in terms of its straggler resilience, and has excellent numerical robustness as long as the workers' storage capacity is slightly higher than the fundamental lower bound. Moreover, it can be decoded using a fast peeling decoder that only involves add/subtract operations. Our second approach has marginally higher decoding complexity than the first one, but allows us to operate arbitrarily close to the lower bound. Its numerical robustness can be theoretically quantified by deriving a computable upper bound on the worst case condition number over all possible decoding matrices by drawing connections with the properties of large Toeplitz matrices. All above claims are backed up by extensive experiments done on the AWS cloud platform.

==> open_issues.tex <==
1. We should check if we use block-columns (with hyphen) consistently throughout.
I think in some places it is not hyphenated.
2. Appendix needs to be re-organized how IEEE journal papers are
3. Need to refer to the finite-field scheme of Yu et al. and show that its performance is quite bad. Need to refer to Li's thesis here.
4. Comparison with R-Tang.
5. At couple of places you have used a very small font for the equations. This is not good. You can move the equation to the top of the page and make it span both columns.
6. Last Appendix on numerical experiments can be moved to numerical experiments section.
7. All code for recreating the experiments needs to be uploaded to appropriate repository.
8. Need to be clear that the worker node computational complexity depends on t but the decoding complexity does not. We can loosely state this and then refer to the SP Mag article.
